The Workflow Trace Archive: Open-Access Data from Public and Private Computing Infrastructures -- Technical Report

Realistic, relevant, and reproducible experiments often need input traces collected from real-world environments. We focus in this work on traces of workflows---common in datacenters, clouds, and HPC infrastructures. We show that the state-of-the-art in using workflow-traces raises important issues: (1) the use of realistic traces is infrequent, and (2) the use of realistic, {\it open-access} traces even more so. Alleviating these issues, we introduce the Workflow Trace Archive (WTA), an open-access archive of workflow traces from diverse computing infrastructures and tooling to parse, validate, and analyze traces. The WTA includes ${>}48$ million workflows captured from ${>}10$ computing infrastructures, representing a broad diversity of trace domains and characteristics. To emphasize the importance of trace diversity, we characterize the WTA contents and analyze in simulation the impact of trace diversity on experiment results. Our results indicate significant differences in characteristics, properties, and workflow structures between workload sources, domains, and fields.

==> 3_requirements.tex <==


\section{Requirements}
\label{sct:wta-requirements}

\todolaurens{AI/RP: Radu did not like the text in Section 3 (requirements) and suggested we cut it significantly. If we do this, we can merge it into Section 4 + drop the claim related to formulating requirements. This has pros and cons, among which I see as benefit having more space for experimental results (analysis/simulation) and the drawback of making the design of the archive seem simpler than what it is. Your choice, yours to implement.}

In this section, we identify five key requirements for the structure, content, and operation of a useful archive for workflow traces.
Requirements 1--3, in particular, focus on the unique nature of workloads comprised of workflows. 


\noindent \textbf{\wtareq{1}: Diverse Traces for Academia, Industry, Education.}

The main findings in Section~\ref{sec:survey:diversity} give strong evidence that the archive must include a diverse set of traces, corresponding to the many existing workflow domains and fields. Moreover, the archive must include traces that cover a broad spectrum of workflow sizes, structures, and other characteristics, including both general characteristics to many domains and fields, and idiosyncratic characteristics corresponding to only one domain or field. 




Addressing this requirement is important.
For academia, experimenting with representative traces increases credibility and demonstrates the applicability of an approach.
To claim generality of a solution, experiments must be conducted using various traces; we give further evidence for this in Section~\ref{sct:validation-and-threats}.
For industry, representative traces are essential to test production-ready systems, and can act as a validation for techniques proposed by academia~\cite{klusavcek2014interactions}.
Furthermore, as systems become more complex, education and training on these topics become ever more important.

\noindent \textbf{\wtareq{2}: A Unified Format for Workflow Traces.} %

To simplify trace exchange, reduce trace integration effort among different systems, prevent double work for other users, and provide dataset independent tools (expressed as \wtareq{3}), the archive must define a unified trace format.
The format 
must cover a broad set of data about the workloads and about the workflow management systemsm including:
workload metadata;
workflow-level data including \glspl{nfr} and common metadata;
task-level data including per-task \glspl{nfr} and operational metadata such as task-state changes;
inter-dependencies between tasks and other operational elements such as data transfers; 
system-level information including resource provisioning, allocation, and consumption; etc.

Preserving such information is challenging, posing a design trade-off between verbosity and meaning. For example, we explicitly require from the format to support per-task \gls{nfr} specification and system-level monitoring. Although workflows already pose complex \glspl{nfr} at both application and task-level, currently no common format exists for expressing them. 
Similarly, although system state monitoring is common in datacenter, cloud, and HPC infrastructures, there currently exists no consensus about the possible monitoring metrics to select~\cite{DBLP:conf/wosp/XiongPZG13} and archive.
Simply selecting to preserve everything is not possible, because workflow data may be sensitive (e.g., in bioinformatics, only basic workflow information can be shared) and system-level data may be overwhelmingly large.



Addressing this requirement is the basis of any data archive. Additionally, a unified trace format for workloads of workflows helps provide the structured provenance information~\cite{7160272} to improve the reproducibility of experimental results.%






\noindent \textbf{\wtareq{3}: Detailed Insights into Trace Properties.}

Simply archiving data is not enough, as it must provide insight into its traces at the level of detail required by the broad audience implied by \wtareq{1}, from beginner to expert.
Additionally, the archive must scale with an increasing number of users and stored data.

Broad insights, easily provided in standardized reports, include {\it extrinsic properties} such the number of workflows and tasks and the number of users in the trace, while {\it intrinsic properties} include the workflow arrival patterns and the resource consumption per-task.

Detailed insights include expert-level {\it analysis of single traces} at workload-, workflow-, and system-level; and {\it collective analysis} across all traces and across traces with a shared feature (e.g., all traces of a domain or field). For each, the archive must support advanced analysis of structural patterns across domains and fields, the burstiness of the arrival pattern in a workload, the maximal level of parallelism and the critical-path length of individual workflows, and so forth. Further examples of such analysis appear in Section~\ref{sct:workflow-characterization}.
These properties must be accessible through readily available tools (see \wtareq{4}) and, possibly, through interactive online reports.

Basic and detailed insights allow the community create a common body of easily verified knowledge. Additionally, practitioners can correlate information across multiple traces, resulting in better quantitative evidence, intuition about otherwise black-box applications, and understanding that helps avoiding common pitfalls~\cite{DBLP:conf/jsspp/FrachtenbergF05}.







\noindent \textbf{\wtareq{4}: Tools for Trace Access, Parsing, Analysis, Validation.}

The most important tool is the online presence of the archive itself.
The archive must further provide tools to parse traces from different sources to the unified format~(see also~\wtareq{2}), to provide insight into traces~(see also~\wtareq{3}), and to {\it validate} common properties (e.g., basic checks that all properties are present, and further correctness checks using domain- and expert-knowledge).
An absence of such tools would lead to users unable to select appropriate traces, validate their properties, and compare them. %



 

The archive should further to aid users in building more sophisticated tools.
We envision here scripts and shareable data as building blocks.
Newly built tools can then be added to the selection of tools so more parties can make use of them (helping with \wtareq{5}).





\noindent \textbf{\wtareq{5}: Methods for Contribution.}

The archive must reflect the continuous evolution of workflow use in practice, by increasing the coverage of different scenarios.
We make a distinction between two types of contribution: 
(1) additional traces, possibly originating from a new domain or application-field, and 
(2) additional traces, introducing new properties.
To facilitate the former contribution, the archive must provide a method for the upload and (basic) automated verification of traces. %
To facilitate the latter, the format must integrate specific provisions that enable upgrades, such as versioning. 


Having methods to contribute new workloads is key to encourage new and existing contributors to submit traces.
In particular, tools to add new domains are of particular importance, to support emerging paradigms with realistic data.
For example, the emerging Function as a Service (FaaS) platforms offer serverless workflows functionality, yet no (public) FaaS workflow trace exists currently.
We foresee FaaS workflows being expressed by our format through using already supported properties such as the \textit{parameters} and \textit{NFRs} dictionaries for e.g. function versioning and locality constraints that may need to be expressed in such workflows.


==> 7_threats_to_validity.tex <==
\section{Threats to validity}

A possible threat to this work is the selection of venues in the survey.
Besides omitting venues that yielded no results on our initial query, we made sure that both journals and conferences were covered at various levels in term of quality.
We believe this covers the field of systems community to a degree where conclusions can be drawn from.

Another threat is the (level of) anonymization of the data.
The Google team published interesting work on the anonymization of data~\cite{clusterdata:Reiss2012}, yet we believe this type of anonymization is not suitable for this work.
Normalizing values of both resource consumption and available resources significantly reduces the usability of traces and the characterization details they provide.
We think obfuscation techniques such as multiplying both consumption and resources by a certain factor, allows for relative comparisons and the possibility to replay scheduling the workload on the resources while still concealing the original data.

A third threat is the diversity of traces. Given the constraints and difficulty of collecting traces, the constituents of the archive offer significant variety. 
The traces have been collected from eight sources, span three domains, and over ten applications. 
They range in size from tens to millions of workflows. 
The workflows themselves have time spans ranging from minutes to days. 
Our introduction of new traces from engineering and industrial domain apart from the popular scientific traces increase the diversity of traces available to the community. 
Our comparative characterization across domains and sources highlights the diversity of traces in the community.

A fourth threat is the properties included in the workload trace format.
While we try to include most properties available, low-level details such as page caches are omitted to not unnecessarily complicate the traces.
If future work demands these needs, the versioning schema per object will allow for these additions.
